Risk-averse model predictive control

Risk-averse model predictive control (MPC) offers a control framework that allows one to account for ambiguity in the knowledge of the underlying probability distribution and unifies stochastic and worst-case MPC. In this paper we study risk-averse MPC problems for constrained nonlinear Markovian switching systems using generic cost functions, and derive Lyapunov-type risk-averse stability conditions by leveraging the properties of risk-averse dynamic programming operators. We propose a controller design procedure to design risk-averse stabilizing terminal conditions for constrained nonlinear Markovian switching systems. Lastly, we cast the resulting risk-averse optimal control problem in a favorable form which can be solved efficiently and thus deems risk-averse MPC suitable for applications.

==> chow-example.tex <==
Here we apply the reformulation presented in Section~\ref{sec:computational} 
on the problem taken from~\cite[Sec. X.A]{chow2017arxiv}. The system is an \ac{mjls} with \(6\) 
modes and ellipsoidal state-input constraints.
Even though the formulation of the \ac{mpc} problem is different, as briefly discussed in 
Section~\ref{sec:markovian_switching_systems},
our reformulation of the optimization problem as a \ac{qcqp} can be readily applied.
Starting at \(x_0=(2.5, 2.5)\) we apply the \ac{mpc} control law
for randomly generated switching paths.
Statistics regarding the time to compute a control action running the 
risk-averse \ac{mpc} are reported in Table~\ref{tbl:chow_solver_time}. 
Runtime scales roughly linearly with the number of scenarios and is 
lower compared to those reported in~\cite{chow2017arxiv}.
Indicatively, for \(N=6\), \cite{chow2017arxiv} reports online computation 
times that exceed \(2\) hours.
All simulations were performed in MATLAB using YALMIP~\cite{Lofberg2004} 
with the MOSEK solver and were executed on 
an Intel i5-6200U CPU at 2.30GHz with 8GB RAM running Ubuntu 16.04.


\begin{table}[ht]%
\begin{minipage}{0.45\linewidth}%
\setlength{\tabcolsep}{4pt}%
\def\arraystretch{1.15}%
 \begin{tabular}%
 {@{}>{\scriptsize}c >{\scriptsize}c >{\hspace*{2.1ex}\scriptsize}l >{\hspace*{1.8ex}\scriptsize}l@{}} 
 \(N\)%
 & scenarios%
 & \multicolumn{1}{c}{\scriptsize mean}% 
 & \multicolumn{1}{c@{}}{\scriptsize max}\\[0.1ex]%
 \hline%
 3  & 216      &  \llap0.02    &  \llap0.08\\%
 4  & 1296     &  \llap0.16    &  \llap0.39\\%
 5  & 7776     &  \llap1.06    &  \llap1.65\\%
 6  & 46656    &  \llap8.47    &  \llap{13}.31\\[0.1ex]%
 \hline%
 \end{tabular}%
\end{minipage}%
\begin{minipage}{0.54\linewidth}%
 \caption{%
  \scriptsize Runtime (in seconds) for different \(N\) on the problem taken 
  from~\cite{chow2017arxiv} for \(\alpha = 0.75\). Average and maximum runtimes are taken
  over \(100\) runs for \(N=3,4,5\) and \(10\) runs for \(N=6\).}%
  \label{tbl:chow_solver_time}
\end{minipage}  
\end{table}
%
%
